Scalable Bicriteria Algorithms for Non-Monotone Submodular Cover

In this paper, we consider the optimization problem \scpl (\scp), which is to find a minimum cost subset of a ground set $U$ such that the value of a submodular function $f$ is above a threshold $\tau$. In contrast to most existing work on \scp, it is not assumed that $f$ is monotone. Two bicriteria approximation algorithms are presented for \scp that, for input parameter $0 < \epsilon < 1$, give $O( 1 / \epsilon^2 )$ ratio to the optimal cost and ensures the function $f$ is at least $\tau(1 - \epsilon)/2$. A lower bound shows that under the value query model shows that no polynomial-time algorithm can ensure that $f$ is larger than $\tau/2$. Further, the algorithms presented are scalable to large data sets, processing the ground set in a stream. Similar algorithms developed for \scp also work for the related optimization problem of \smpl (\smp). Finally, the algorithms are demonstrated to be effective in experiments involving graph cut and data summarization functions.

==> sections/theoretical/stream2_pseudo.tex <==
\begin{algorithm}[tb]
\caption{\streampar}\label{alg:stream2}
\textbf{Input}: $\guess$, $\epsilon$\\
\textbf{Output}: $S\subseteq U$
\begin{algorithmic}[1]
  \STATE $S_1\gets\emptyset,...,S_{\smallpb}\gets\emptyset$
  \FOR {$u$ received from stream such that $w(u)\leq\guess$}
    \IF {$\exists j$ s.t.
         $\Delta f(S_j,u)/w(u)\geq \epsilon \tau/(2 \guess)$}
         \STATE $S_j\gets S_j\cup\{u\}$
         \IF{$w(S_j) > 2 \guess/\epsilon$}\label{line:full}
         \STATE \textbf{break}
         \ENDIF
    \ENDIF
  \ENDFOR
  \STATE $S_0\gets$\uncons$\left(\cup_{j=1}^{\smallpb}S_j\right)$\label{line:uncons}
  \STATE \textbf{return} $\argmax\{f(S_0),...,f(S_{\smallpb})\}$\label{line:complete}
  %\If {$\max\{f(S_0),...,f(S_{\smallpb})\}\geq \alpha(1-\epsilon)\tau$}\label{line:end}
  %  \State \textbf{return} $\argmax\{f(S_0),...,f(S_{\smallpb})\}$
  %\EndIf

\end{algorithmic}
\end{algorithm}


==> sections/theoretical/stream_theorem.tex <==
\begin{lemma}
  %\label{lemma:streamratio}
  Suppose that \stream is run with $\guess\geq OPT$.
  Let $S$ be the set returned by \stream.
  Then $f(S)\geq\gamma (1-\epsilon)\tau$.
\end{lemma}
\begin{proof}
  The loop on Line \ref{line:loop} of \stream completes in one of two ways:
  (i) The if statement on Line \ref{line:full} has been satisfied;
  or (ii) All of the elements of $U$ have been read from the stream, and Line
  \ref{line:full} was never satisfied.
  The proof of Lemma \ref{lemma:streamratio} is broken up into each of these two
  events.

  First suppose event (i) above occurs.
  Then at the completion of the loop there exists some $r\in\{1,...,\smallpb\}$ such that
  $w(\Si{r})\geq\maxsize$. Let $\Si{r}(\ell)$ be $\Si{r}$ after the $\ell th$ element
  was added to it and $\Si{r}(0)=\emptyset$. Then at the completion of \stream
  \begin{align*}
    f(\Si{r}) &\overset{(a)}{\geq} f(\Si{r})-f(\emptyset) \\
    &= \sum_{\ell=1}^{|\Si{r}|}\left(f(\Si{r}(\ell))-f(\Si{r}(\ell-1))\right) \\
    &\overset{(b)}{\geq} \sum_{x\in \Si{r}}\gain \\
    &= w(\Si{r})\epsilon\tau/(2\guess) \\
    &\overset{(c)}{\geq} \tau
  \end{align*}
  where (a) is because $f(\emptyset)\geq 0$; (b) is by the condition on Line \ref{line:add}; and
  (c) is by the assumption that $w(\Si{r})\geq\maxsize$.
  Therefore at the completion of \stream
  $\max\{f(\Si{0}),...,f(\Si{\smallpb})\}\geq f(\Si{r})\geq \tau.$

  Now suppose that event (ii) above occurs.
  Then at the end of \stream, $w(\Si{j})<\maxsize$ for all $j\in\js$.
  For this case, we need the following claim which is proven in the appendix,
  and is based on a result from \citet{feige2011maximizing}
  which is stated as Lemma \ref{lemma:expected} in the appendix.
  \begin{claim}
    %\label{claim:mono}
    Let $A_1,...,A_m\subseteq U$ be disjoint, and $B\subseteq U$.
    Then there exists $i\in\{1,...,m\}$ such that
    $f(A_i\cup B)\geq (1-1/m)f(B)$.
  \end{claim}
  Let $S^*$ be an optimal solution to the instance of \scp.
  By Claim \ref{claim:mono}, there exists $t\in\{1,...,\smallpb\}$ such that
  $(1-\epsilon/2)\tau\leq f(S^*\cup S_t)$.
  Define $\opta=S^*\cap (\cup_{i=1}^{\smallpb}S_i)$ and
  $\optb=S^*\setminus \opta$.
  Then,
  \begin{align}
    (1-\epsilon/2)\tau &\leq f(S^*\cup S_t) \nonumber \\
    &= f(\opta\cup S_t) + f(S^*\cup S_t) - f(\opta\cup S_t) \nonumber\\
    &\overset{(a)}{\leq} f(\opta\cup S_t) +\sum_{x\in \optb}\Delta f(\opta\cup S_t, x)\nonumber\\
    &\overset{(b)}{\leq} f(\opta\cup S_t) +\sum_{x\in \optb}\Delta f(S_t, x)\label{eqn:1}
  \end{align}
  where (a) and (b) are both due to submodularity. In addition,
  \begin{align}
    \sum_{x\in \optb}\Delta f(S_t, x) &\overset{(a)}{<} \sum_{x\in \optb}\gain \nonumber \\
    &= w(\optb)\epsilon\tau/(2\guess)\nonumber \\
    &\overset{(b)}{\leq} w(\optb)\epsilon\tau/(2OPT)\nonumber \\
    &\overset{(c)}{\leq} \epsilon \tau/2\label{eqn:327}
  \end{align}
  where (a) is by submodularity and the condition on Line \ref{line:add};
  (b) is because $\guess\geq OPT$;
  (c) is because $\optb\subseteq S^*$ implies that $w(\optb)\leq OPT$.
  Then by combining Inequalities \ref{eqn:1} and \ref{eqn:327}, we have that
  \begin{align*}
    (1-\epsilon)\tau &\leq f(\opta\cup S_t)\\
    &\overset{(a)}{\leq}\max_{Y\subseteq \cup_{i=1}^{\smallpb}S_i}f(Y)\\
    &\overset{(b)}{\leq} \frac{1}{\gamma}f(\Si{0})
  \end{align*}
  where (a) is because $\opta\cup S_t\subseteq \cup_{i=1}^{\smallpb}S_i$;
  (b) is because $\Si{0}$ is an $\gamma$-approximate maximum of $f$ over
  $\cup_{i=1}^{\smallpb}\Si{i}$.
  Therefore $\max\{f(\Si{0}),...,f(\Si{\smallpb})\}\geq f(\Si{0})\geq \gamma(1-\epsilon)\tau.$
\end{proof}

















%


==> sections/todo.tex <==
Alan: Check impossibility results?

TODO: Define bicriteria, check the statement of feige et al., discussion of how we
know what to set $\tau$ to, can we use this alg for unconstrained?, check bilmes
result, feasibility guarantee.

Why bicriteria approximation algorithms are useful.

TODO: Discuss how cost is both for memory as well as cost of solution.

Time is in queries of $f$

Define weight of a set, delta notation.

TODO: Give intuition about why we need a bunch of disjoint sets.

TODO: Define $OPT$ in problem definition, talk about using randomized unconstrained
approximation algorithms, define constraint approximation, figure out
total number of queries, define $w_{min}$, change $\epsilon$ to $\delta$?,
look for that paper on knapsack streaming.

How novel is Claim 1? Are we citing the correct claim?

Why does multi make increasingly large guesses?

Define $w_{min}$

TODO: Queries per received element? Impossibility result from other cover
streaming paper, instance notation, write below impossibility result as a formal
statement.

Intuition for the impossibility of single pass.

Analyze run times!

How can you get an upper bound on OPT?

More discussion before each theoretical guarantee? The memory of single pass.
How at first limited by elements being read in, quickly find feasible,
then limited by competitive ratio.

Instead of appendix, just say proof is in the detailed version of the paper.

Running unconstrained periodically or after every element?

Is bimax actually a streaming algorithm?

Write for each proof in appendix.

Talk about using probabilistic algorithms for USM.

Define USM

TODO: How can you pick $\tau$ that satisfies the definition? Justify cover version
of the problem.

TODO: Problem acronyms.

TODO: Submodular threshold instead of submodular cover?

TODO: Particular number of guesses bilmes makes for optimum? Run time?

TODO: Is norouzi really in the streaming setting? What is the memory for the multipass?

TODO: In-depth discussion how this is related to alaluf, norouzi, etc.. We don't have to
deal with too many elements the way that alaluf does.

TODO: Experimental section put run time, guarantee, etc..

TODO: How are SG and ALALUF the most scalable?

Another way of looking at all this is that I made a 1/2 approx algorithm for
submodular maximization, and using the bilmes approach for cover.

max memory = stored cost

In experiments describe how algorithms compare to the unconstrained algorithm.

TODO: Check the total number of queries

Computations for each arriving element?

What is something like the greedy algorithm were analyzed for its number of passes?

Don't totally understand the monotone SC streaming paper's guarantees.

Point out there doesn't exist any USM algorithms for streaming.

Why did you switch datasets in the experiments?

Similar patterns on different datasets can be found in the appendix.

Can view as cost efficient version of unconstrained algorithm.

Example showing that unconstrained has no guarantee.

Why compare to DG?

"cost memory"

parameter table

how is the max alg different from just using the approach of bilmes

what happens to the impossibility results if tau is beneath the max value? What
happens if you just run unconstrained.

Impossibility results for maximization? Can we get a ratio better than that?

Is that Nemhauser paper about knapsack constraint?

Be careful about cardinality vs knapsack constrained submodular maximization. Make
it clear which case.

Define USM

Difference between multi and single is how the guesses of opt are (sequential or parallel)

Is bimax the same approach as Bilmes?

multi makes one more pass to find the min cost.

"Memory cost"

ground set instead of input set?

nln(n) should be nln(OPT)

Single pass time should be per element + post processing?

Why B?

Emphasize in stream guess of OPT.

Dynamic unconstrained, random set approach?

Tradeoff between cost and feasibility

Need competitive ratio since bound B may be bad

ln to log

Section name don't just have algorithm

More details about algs input

Put special memory part in the contributions

Precedent for $B$.

